Consistent cosmic shear in the face of systematics: a B-mode analysis of KiDS-450, DES-SV and CFHTLenS

We analyse three public cosmic shear surveys; the Kilo-Degree Survey (KiDS-450), the Dark Energy Survey (DES-SV) and the Canada France Hawaii Telescope Lensing Survey (CFHTLenS). Adopting the COSEBIs statistic to cleanly and completely separate the lensing E-modes from the non-lensing B-modes, we detect B-modes in KiDS-450 and CFHTLenS at the level of about 2.7 $\sigma$. For DES- SV we detect B-modes at the level of 2.8 $\sigma$ in a non-tomographic analysis, increasing to a 5.5 $\sigma$ B-mode detection in a tomographic analysis. In order to understand the origin of these detected B-modes we measure the B-mode signature of a range of different simulated systematics including PSF leakage, random but correlated PSF modelling errors, camera-based additive shear bias and photometric redshift selection bias. We show that any correlation between photometric-noise and the relative orientation of the galaxy to the point-spread-function leads to an ellipticity selection bias in tomographic analyses. This work therefore introduces a new systematic for future lensing surveys to consider. We find that the B-modes in DES-SV appear similar to a superposition of the B-mode signatures from all of the systematics simulated. The KiDS-450 and CFHTLenS B-mode measurements show features that are consistent with a repeating additive shear bias.

==> Results.tex <==
\label{sec:Results}

In this section we show the effect of the systematics explained in \sect\ref{sec:Systematics} on mock data using the statistics explained in \sect\ref{sec:Method}. We also show E/B-mode measurements for the data listed in \sect\ref{sec:Data} and compare that to the mock systematics. Finally, we show the effect of these systematics on a cosmological analysis using CCOSEBIs.
% {\color{red} have to change the covariance gray regions for the mock plots.}

\subsection{Effect of systematics on mock data}

 
Before applying the systematic effects on the mock data we first measure $\xi_\pm$, $\xi_{\rm E/B}$ and COSEBIs for the noise free mocks (see \sect\ref{sec:Systematics} for a brief introduction to the mock catalogues). \fig\ref{fig:MockvsTheory} shows a comparison between measured statistics from 10, noise free, lines of sight (LOS) in SLICS mocks and our theoretical prediction for the input cosmology (see \tab\ref{tab:CosmoParam}) and redshift distribution of galaxies. For the theory we assume a flat $\Lambda$CDM model with a primordial power-law matter power spectrum and \cite{smith03} halofit for the non-linear scales. We use \cite{BondEfstathiou84} transfer function to estimate the linear matter power spectrum. This combination of methods, although dated, was chosen for the comparison as they fit the mocks better than their alternatives. Nevertheless, we see that the theory does not predict the simulated values perfectly. This is partly due to the fact that we only use 10 LOS for our measurements. 

In \fig\ref{fig:MockvsTheory} the grey lines show the estimated value for one LOS, which show a considerable scatter, especially for larger angular scales where the cone size of the ray-tracing becomes important. Even with a larger number of LOS we do not expect the theory to match the mocks perfectly as was demonstrated in  \cite{Harnois15}. On the left panel we show,  $\xi_\pm$ and $\xi_{\rm E/B}$. The top panel shows $\xi_+$ and $\xi_{\rm E}$ in magenta squares and blue diamonds,  respectively. Recall that for a B-mode free data set, $\xi_+=\xi_{\rm E}$. Here we see that at larger angular scales $\xi_{\rm E}$ is smaller than $\xi_+$ and looking at the bottom panel we see that  $\xi_{\rm B}$ is non-zero for the same angular ranges. Although, not shown here, there is a small level of COSEBIs B-modes in the mocks, but its amplitude is two orders of magnitude smaller than the E-mode signal. The bottom left panel in \fig\ref{fig:MockvsTheory} shows $\xi_-$ and $\xi_{\rm B}$ in green + and black x. The theoretical predictions for $\xi_\pm$ are shown as solid magenta and green dashed curves. The right panels  belong to E-mode COSEBIs. Although COSEBIs modes are discrete we connect them together in the plot for visual aid. The black + signs show the theoretical predictions while the blue squares show the mean measured values. Each panel shows $E_n$ for a given angular range, written in the top right corner of the panel. By comparing the left and right panels we can already see that small or large scale biases that can affect 2PCFs, have a minimal effect on COSEBIs. The reason for the robustness of COSEBIs comes from the weight functions that convert shear power spectra to $E_n$ \citep[see figure 4 in][for a comparison between the kernels corresponding to COSEBIs and 2PCFs]{Kilbinger17}. These weights reach zero at low  and diminish at high $\ell$-modes. 

After testing the validity of our raw mock data estimates, we go on to apply the systematics to the data and measure their effect by comparing it to the raw values. As mentioned in \sect\ref{sec:Systematics} some of the systematics have no redshift dependence while the others do, therefore, we divide the results into two subsections. 
 
\subsubsection{Redshift independent systematics}
 
 
\begin{figure*}
   \begin{center}
     \begin{tabular}{c}
     \resizebox{155mm}{!}{\includegraphics{plots/xiEB_2PCFs_Mixed_nThetabins50.pdf}}
     \end{tabular}
   \end{center}
     \caption{\small{The effect of redshift independent systematics on  $\xi_\pm$ and $\xi_{\rm E/B}$. The y-axes for the the left panels show the fractional difference between the  systematic and fiducial cases and for the right panels show the difference between the two times angular distance in arcminutes scaled by $10^4$. Each curve shows the average values for 10 noise free LOS of SLICS mocks with galaxy number density and redshfit distribution of KiDS-450. The left panels show $\xi_+$ in magenta squares and $\xi_-$ in green + signs, while the right panels show $\xi_{\rm E}$ in blue diamonds and $\xi_{\rm B}$ in black x signs. In addition, $\xi_{\rm E}-\xi_{\rm B}$ is shown in red pluses. The grey shaded area in the right panels show the expected error for KiDS-450 data that arises from the noise only terms. Each row of panels show the results for a different systematic effect denoted on the top of the left panels. $\theta$ is divided into 50 logarithmic bins between $0.5'$ and $300'$. }}
     \label{fig:2PCFSys}
 \end{figure*}
 

\begin{figure*}
   \begin{center}
     \begin{tabular}{c}
     \resizebox{160mm}{!}{\includegraphics{plots/MockSysEnBn_1Bin.pdf}}
     \end{tabular}
   \end{center}
     \caption{\small{The effect of redshift independent systematics on  COSEBIs. The full angular range considered here is $[0.5',100']$. We also divide this range into a large and small scale regime of $[40',100']$ and $[0.5',40']$. The y-axis shows the mean difference between the systematic induced mocks and their fiducial values for 10 LOS. The blue squares show the results for PSF-leakage, the green triangles belong to the random correlated noise at chip scale, magenta diamonds show the same systematic for pointing scale correlations and the black stars represent the regular pattern systematic. The left panels show E-modes, while the right ones show B-modes. The x-axis shows the COSEBIs mode, $n$, which is a natural number, however, we connect the points for visual aid. The grey regions show the one sigma, noise only errors, corresponding to KiDS-450 data. }}
     \label{fig:COSEBIsSys}
 \end{figure*} 
 
The redshift independent systematics are the first three effects described in \sect\ref{sec:Systematics}: PSF leakage, random correlated noise per pointing (RCNP) and regular repeating pattern. \fig\ref{fig:2PCFSys} shows a comparison between the mocks affected by the systematics and the fiducial mocks for the traditional statistics, $\xi_\pm$ and $\xi_{\rm E/B}$. The left panels show the ratio of 
$\xi_\pm$ and $\xi_{\rm E}$ to their fiducial values for each systematic, while the right panels show the difference between 
$\xi_{\rm B}$ and its fiducial value as well as $\xi_{\rm E}-\xi_{\rm B}$ for each case. The right panels show the difference since the ratio can blow up as the fiducial $\xi_{\rm B}$ is very small for many angular scales. If a systematic adds to both E/B-modes equally then $\xi_{\rm E}-\xi_{\rm B}=0$ and $\xi_-=0$, however we see that for these systematics that is not the case, especially for larger angular scales. This figure uses the same symbols and colors as \fig\ref{fig:MockvsTheory} with additional red + symbols corresponding to $\xi_{\rm E}-\xi_{\rm B}$. Each row shows the results for the systematic denoted in the top right corner. The grey regions in the right panels show the level of noise expected for KiDS-450 data. Here we use 50 logarithmic $\theta$-bins, to show the effect of systematics in more detail.
 

\begin{figure*}
   \begin{center}
     %\begin{tabular}{c}
     \resizebox{170mm}{!}{\includegraphics{plots/CCOSEBIs_sensitivity_0p50-100.pdf}}
     %\end{tabular}
   \end{center}
     \caption{\small{CCOSEBIs sensitivity to $\Sigma_8$ and systematics E/B-modes for $\theta\in[0.5',100']$. The left panel shows the E-mode CCOSEBIs for 5 modes, $E_{\sigma_8}$ (solid red), $E_{\Omega_{\rm m}}$ (dot-dashed blue), $E_{\sigma_8\sigma_8}$(dashed green), $E_{\sigma_8\Omega_m}$ (solid magenta, bottom curve) and $E_{\Omega_{\rm m}\Omega_{\rm m}}$ (dotted  black) versus $\Sigma_8=\sigma_8(\Omega_{\rm m}/0.3)^{0.65}$. The right panel shows the CCOSEBIs B-modes for the same parameter combinations with each mode indicated in the x-axis. The curves show the theoretical value of E-mode CCOSEBIs using KiDS-450 noise only covariance matrix and redshift distribution.  CCOSEBIs values corresponding to the mocks  are plotted as symbols. The red circles show the fiducial values, green triangles show chip scale random correlated noise, magenta diamonds show pointing scale random correlated noise, blue squares correspond to the PSF leakage systematic and black stars show CCOSEBIs for the regular pattern. The grey region in the left panel roughly shows the one sigma error for $\Sigma_8$ from KiDS-450 cosmic shear analysis, centred on the fiducial values. Moreover, the one sigma errors for a noise only B-mode measurement for KiDS-450 is shown in the right panel as the grey region. Note that the simulations are shape noise free.}}
\label{fig:CCOSEBIsSys}
 \end{figure*}

With the traditional statistics the binning and the assumptions that go into their definition can limit the analysis. Therefore, here we investigate the effect of the systematics using COSEBIs. \fig\ref{fig:COSEBIsSys} shows the relative effect of systematics on E/B-mode COSEBIs, as the difference between their fiducial values and the ones estimated from systematic induced mocks. As before, we show three angular ranges: $[0.5',40']$, $[40',100']$ and $[0.5',100']$, corresponding to small, large and the full angular range, indicated at the top right corner of each panel. The blue squares represent PSF leakage, green triangles and magenta diamonds show random noise correlated at chip scale and pointing scale, respectively and finally the black stars correspond to the regular pattern systematic. All values are shown for the mean of the LOS discussed earlier. The grey regions show the level of noise corresponding to KiDS-450 survey (no cosmic variance term added here). RCNP at chip level shows very small deviations from the fiducial values in agreement with \fig\ref{fig:2PCFSys}. PSF leakage and RCNP at pointing level have a similar effect for lower COSEBIs modes, however, PSF leakage due to its more smooth nature vanishes faster that RCNP at pointing scale, which can allow us to distinguish between these two effects. Regular pattern has a more chaotic effect on COSEBIs. Overall there is more smaller scale changes in the correlation functions for this effect which are picked up by the higher COSEBIs modes and can also be seen in the erratic changes of 2PCFs in \fig\ref{fig:2PCFSys}. For all four systematics, the effects are stronger when the full angular range is used, as can be seen in the middle panels. Comparing the right and left panels we see that all systematics affect both E/B-modes and in some cases E-modes are affected even more substantially. But in general a significant E-mode signal translates to a significant B-mode, which can be used to diagnose the data and then go back to the lower level products and correct for these effects. Alternatively, some of the better known effects can be modelled and corrected at the 2 point statistic level.


Although we can see the signature of each systematic on COSEBIs in \fig\ref{fig:COSEBIsSys}, it is not clear if they have any effect on cosmological parameters. Which is why we use compressed COSEBIs to investigate the existence of such effects. Note that one could instead do a likelihood analysis to find any biases introduced by these systematics. On the other hand, using CCOSEBIs provides us with a short-cut, as they are formed of linear combinations of COSEBIs that are sensitive to cosmological parameters. Here we focus on $\Sigma_8=\sigma_8(\Omega_{\rm m}/0.3)^\alpha$, as this is the combination of parameters that cosmic shear data is mostly sensitive to. We find that for a KiDS-450 redshift distribution $\alpha=0.65$ best describes the degeneracy direction (see \App\ref{app:CCOSEBIs}).  Because we are only interested in $\Sigma_8$ we only consider first order CCOSEBIs for $\sigma_8$, $\Omega_{\rm m}$ (based on first order derivatives with respect to the parameter), and second order ones for $\sigma_8 \sigma_8$, $\sigma_8\Omega_{\rm m}$ and $\Omega_{\rm m}\Omega_{\rm m}$ (based on second order derivatives with respect to the parameters). Although it is possible to construct a CCOSEBIs mode that is sensitive to $\Sigma_8$ directly, we choose to look at the 5 modes mentioned above which allow an internal consistency check as we will see shortly. For this task we first map each CCOSEBIs to a  $\Sigma_8$ using our theory pipeline and then over plot the values found from simulations. The left panel in \fig\ref{fig:CCOSEBIsSys} shows the results. Each curve shows how a CCOSEBIs E-mode changes with respect to $\Sigma_8$ for the total angular range of $[0.5', 100']$. The CCOSEBIs modes are constructed using KiDS-450 noise covariance and redshift distribution. Note that as was mentioned in \sect\ref{sec:Method} the first few COSEBIs modes contain almost all of the relevant cosmological information, hence CCOSEBIs modes are mainly sensitive to these modes, therefore, any high order COSEBI mode signal is not captured by the CCOSEBIs.

In \fig\ref{fig:CCOSEBIsSys} the curves from top to bottom correspond to the CCOSEBIs modes that based on derivative with respect to $\sigma_8\sigma_8$, $\Omega_m\Omega_m$, $\sigma_8$, $\Omega_{\rm m}$ and $\sigma_8\Omega_{\rm m}$. Each symbol corresponds to one of the systematic cases, aside from the red circles which show the values for the fiducial mocks. The grey region shows the error on $\Sigma_8$ centered on the red circles, taken from KiDS-450 data analysed in \cite{hildebrandt/etal:2017}. We can see that all the systematics increase the value of $\Sigma_8$, with regular pattern having the largest effect. We can also see that in some cases the symbols do not line up, with each CCOSEBIs mode corresponding to a different $\Sigma_8$. This can potentially be used in data analysis as another tool for diagnosing systematics. The right panel of \fig\ref{fig:CCOSEBIsSys} shows the B-mode CCOSEBIs for each case on the left panel. We expect B-modes to be zero in the absence of systematics and astrophysical effects. We see that the fiducial mocks have a very small residual B-mode, also seen with the other methods. The grey region in the right panel shows the error for noise only B-modes for KiDS-450 data. A comparison between the two panels reveals a close connection between E/B-modes. Mainly that a larger bias in E-modes corresponds to a larger B-mode and that both residuals are positive. Note that this conclusion does not necessarily hold for all angular ranges. For example, for the large scales, $E_1$ and $E_2$, which contain most of the cosmological information, are negative as can be seen in \fig\ref{fig:COSEBIsSys} (see \fig\ref{fig:MockvsTheory} for the fiducial values), which does not fit any standard cosmological model. This shows that although the large scales have the lowest signal to noise, they can be used as an investigative tool for hunting systematics in the data. 


\subsubsection{Redshift dependent systematics}
\label{sec:resultZdep}
 
 
\begin{figure*}
   \begin{center}
     \begin{tabular}{c}
     \resizebox{150mm}{!}{\includegraphics{plots/xiEB_2PCFs_VariableDepth_Mixed_nThetabins50.pdf}}
     \end{tabular}
   \end{center}
     \caption{\small{The effect of variable depth systematic on  $\xi_\pm$ and $\xi_{\rm E/B}$ for a single redshift bin. The y-axis is the difference between the measurements for the variable and uniform depth cases times angular distance in arcminutes. Each curve shows the average values for 30 noise free LOS of SLICS mocks. The left panels show $\xi_+$ in magenta squares and $\xi_-$ in green '+' signs, while the right panels show $\xi_{\rm E}$ in blue diamonds and $\xi_{\rm B}$ in black 'x' signs. In addition, $\xi_{\rm E}-\xi_{\rm B}$ is shown in red pluses. $\theta$ is divided into 50 logarithmic bins between $0.5'$ and $300'$. The grey region shows the one sigma error for KiDS-450 data. The plots are zoomed in to show the effect of this systematic clearly. See \fig\ref{fig:2PCFSys} for the full size of the errorbars. }}
     \label{fig:var1bin}
 \end{figure*}
 
  \begin{figure}
   \begin{center}
     \begin{tabular}{c}
     \resizebox{70mm}{!}{\includegraphics{plots/MockSysCOSEBIs_VariableDepth_diff_1Bin.pdf}}
     \end{tabular}
   \end{center}
     \caption{\small{The effect of variable depth systematic on COSEBIs for a single redshift bin. The y-axis shows the difference between COSEBIs for variable and uniform depth.The blue diamonds correspond to E-modes and the black + signs show B-modes. The grey region shows the one sigma error for a Euclid like survey. These three angular ranges are shown: $[0.5',40']$, $[0.5',100']$ and $[40',100']$.}}
     \label{fig:varCOSEBIs1bin}
 \end{figure}  
 
In \sect\ref{sec:sysZdep} we introduced two systematics that can affect galaxies based on their redshift. In this section we first show results  for the variable depth systematic explained in \sect\ref{sec:sysVariableDepth} and then for the redshift and PSF correlation introduced in \sect\ref{sec:sysZPSF}. 

\subsubsection*{Variable Depth}

\fig\ref{fig:var1bin} shows a comparison between the variable and uniform depth 2PCFs and $\xi_{\rm E/B}$ for a single redshift bin. Here we zoom in the plot to show the subtle effect of the variable depth in KiDS-450 data. See \fig\ref{fig:2PCFSys} for the full KiDS-450 errorbars shown as the grey shaded regions. For the angular scales considered in this paper the difference between uniform and variable depth is at most a few percent for $\xi_+$. However, for $\xi_-$ it can have a larger effect at small angular ranges. \fig\ref{fig:var1bin} shows that there is excess correlation at angular ranges well within the pointing level which is then compensated by a loss of correlation at around the pointing scale. Above that scale the behaviour of the 2PCFs becomes erratic. The exact pattern seen here is sensitive to the relative position of different pointings. Hence to correct for this effect it is important to reproduce the exact depth pattern of the data. 
 
\fig\ref{fig:varCOSEBIs1bin} shows the variable depth effect on COSEBIs. The grey shaded regions correspond to a Euclid-like survey. We can see that for the smaller angular range which is within a pointing level, only low n-modes are affected, however for the full range of $[1',100']$ higher n-modes are also affected. Another signature of this systematic is that it affects E-modes much more significantly than B-modes. But on the plus side it is in practice simpler to model and correct for in the data. 
 
 
 \begin{figure*}
   \begin{center}
     \begin{tabular}{c}
     \resizebox{160mm}{!}{\includegraphics{plots/xiEB_2PCFs_VariableDepth_Mixed_nThetabins50_4bins.pdf}}
     \end{tabular}
   \end{center}
     \caption{\small{The effect of variable depth systematic on  $\xi_\pm$ and $\xi_{\rm E/B}$ for tomographic redshift binning. The y-axis is the difference between the measurements for the systematics case and the fiducial ones times angular distance in arcminutes. Each curve shows the average values for 30 noise free LOS of SLICS mocks. The top right panels show $\xi_+$ in magenta squares and $\xi_-$ in green + signs, as well as $\xi_{\rm E}$ in blue diamonds the bottom right panels show $\xi_{\rm B}$ in black x signs and $\xi_{\rm E}-\xi_{\rm B}$ is shown in red pluses. $\theta$ is divided into 50 logarithmic bins between $0.5'$ and $300'$. The grey region shows the one sigma error for KiDS-450 data. The plots are zoomed in to show the effect of this systematic clearly. {\color{red} move to appendix?} }}
     \label{fig:var4bins}
 \end{figure*} 
 
Figures \ref{fig:var4bins} and \ref{fig:varCOSEBIs4binAll} show the effect of the variable depth when tomography is involved. Each panel shows the results for a pair of redshift bins, denoted at the top of panel, with $z=4$ as the highest redshift bin. \fig\ref{fig:var4bins} shows the fractional difference between the variable and uniform distributions on the top triangle for $\xi_\pm$ and $\xi_{\rm E}$, while the bottom panels swho the difference between the two for $\xi_{\rm B}$ and $\xi_{\rm E}-\xi_{\rm B}$. The grey region corresponds to KiDS-450 errorbars, however, as before the plots are zoomed in.
% an the full error size can be seen in \fig\ref{fig:XiPSFz}. 
On the other hand \fig\ref{fig:varCOSEBIs4binAll} shows the difference between the variable and uniform depth $E_n$ and $B_n$ on the top and the bottom triangles, respectively. The grey regions in \ref{fig:varCOSEBIs4binAll} correspond to a Euclid-like survey. This figure shows the changes
in a more absolute sense, compared to figure \ref{fig:var4bins}, where relative differences are shown for the top triangle\footnote{Since $E_n$ goes to zero at larger n-modes for a systematic free data-set we cannot show the full range of E-modes as a fractional difference}. We see that variable depth has the largest effect on the highest redshift bin, seen both as E and B modes. However, the relative changes caused by this systematic affect all redshift bins at a similar level (see figure \ref{fig:var4bins}).

  \begin{figure*}
   \begin{center}
     \begin{tabular}{c}
     \resizebox{160mm}{!}{\includegraphics{plots/MockSysEnBn_VariableDepth_diff_4Bins0p5_100_EuclidErrors.pdf}}
     \end{tabular}
   \end{center}
     \caption{\small{The effect of variable depth systematic on COSEBIs for tomographic binning for the angular range of $[0.5',100']$. The top right panels show E-modes, and the bottom left belong to B-modes. The grey shaded region shows the one sigma error region for a Euclid-like survey. Each panel shows the results for the redshift bin pair indicated in the panel. }}
     \label{fig:varCOSEBIs4binAll}
 \end{figure*}
 
 
 
 
 \subsubsection*{PSF-z}
 
 \begin{figure*}
   \begin{center}
     \begin{tabular}{c}
     \resizebox{160mm}{!}{\includegraphics{plots/xiEB_2PCFs_PSFz_AllGalsNoZCuts_test4_constantPSFperPointing_nThetabins9_1bin.pdf}}\\
     \resizebox{160mm}{!}{\includegraphics{plots/xiEB_2PCFs_PSFz_test4_constantPSFperPointing_nThetabins9_1bin.pdf}}
     \end{tabular}
   \end{center}
     \caption{\small{2PCFs and $\xi_{\rm E/B}$ for PSF-z systematic. The top two panels show the results when all the galaxies are considered (no redshift cuts), while the bottom two demonstrate the effect of a redshift cut. The left panels show $\xi_\pm$ in magenta squares and green plus signs, respectively. The right panels show $\xi_{\rm E/B}$ and the difference between the two in blue diamonds, black crosses and red plus signs, respectively. The errorbars correspond to the level of ellipticity noise in the mock data. }}
     \label{fig:PSFz2PCFs}
 \end{figure*}
 
 
 \begin{figure*}
   \begin{center}
     \begin{tabular}{c}
     \resizebox{160mm}{!}{\includegraphics{plots/COSEBIs__test4_constantPSFperPointing__4Bins_nMin1_nMax_20_0p50-100p00.pdf}}
     \end{tabular}
   \end{center}
     \caption{\small{ COSEBIs E/B-modes for PSF-z systematic for $\theta\in[0.5', 100']$. The top triangle shows E-modes in red diamonds and the bottom triangle shows B-modes in black pluses. The errorbars correspond to the mock data. Each panel shows COSEBIs for a redshift bin pair denoted at the corner of the panel, with z$_ij$ corresponding to the correlation between redshift bins $i$ and $j$. COSEBIs modes are discrete and here we join them together for visual aid. The mocks used here care noise only and the signal is produced via the correlation between PSF and redshift binning.}}
     \label{fig:PSFzCOSEBIs4bins}
 \end{figure*}
 
 
 
The modelling of this systematic is explained in \sect\ref{sec:sysZPSF}, here we show the effects of this systematic on two point statistics. Starting with the traditional statistics in \fig\ref{fig:PSFz2PCFs}, we compare two cases. The top panels show 2PCFs for no redshift cuts (all of the galaxies are used in the analysis), whereas the bottom panels show the same for a redshift cut of $0.1\leq z_{\rm B}\leq 0.9$. The left panels show $\xi_\pm$ in magenta squares and green + signs, respectively. $\xi_{\rm E}$, $\xi_{\rm B}$ and their difference is shown on the right panels, as blue diamonds, black x symbol and red + signs. Nine logarithmic angular bins are used in these plots. The y-axis shows a 2PCF multiplied by $\theta$ in arcminutes and scaled by $10^4$. The errorbars show one sigma errors for the mock data.  
 
Comparing the two cases in \fig\ref{fig:PSFz2PCFs} we immediately see that the redshift cut has produced a signal. Note that the mock data used here is consistent with noise and should contain no signal. We can see that the signal on the top panels is consistent with zero, while specially the $\xi_+$ signal is highly non-zero. Since the level of $\xi_-$ is small, we can assume that this systematic produces similar levels of E/B-modes, which is roughly shown on the right panel as the difference between $\xi_{\rm E}$ and  $\xi_{\rm B}$ which is near zero for smaller angular ranges. 
 
To see the full effect of the correlation between PSF and redshift binning, we use four redshift bins corresponding to KiDS-450 data and measure COSEBIs on the mock data. \fig\ref{fig:PSFzCOSEBIs4bins} shows the results, with p-values which quantify the significance of this effect. We assume zero signal in the mocks and use a theoretical covariance to estimate a $\chi^2$ value for COSEBIs and then calculate the p-value corresponding to that $\chi^2$. A smaller than $0.01$ p-value ($\sim 2.5\sigma$) is usually considered as a good indication of the failure of the null hypothesis (here zero signal is the null hypothesis). The p-values in the figure are however much smaller than that ($\sim 20\sigma$), hence there should be very little doubt in the existence of this signal. As in \fig\ref{fig:PSFz2PCFs} we see that the E/B-modes are rather similar specially for the lower n-modes and both E/B-modes are larger for the highest redshift bins. 

We summarize the p-values for COSEBIs for all cases in \tab\ref{tab:pvaluePSFz}. The p-values are shown for both E/B-modes for three cases shown in separate rows: no redshift cuts, single bin cut and 4 redshift bins. Each column belongs to a different angular range, corresponding to the three angular ranges that we have used throughout the paper. We see that the no z-cuts cases show no signal as expected, while any redshift cut produces a signal where there should be none. However for the setup we have used the lower angular range shows no signal. The full angular range of $[0.5', 100']$ shows a very significantly non-zero signal, whereas the highest angular range shows much less significance. We also see that increasing the number of redshift bins amplifies the effect. For example for $[40',100']$ the p-values are above the $1\%$ level for the single z-bin case, however with 4 redshift bins they become significant.   
  
  
 
 
\begin{table}
\centering
\caption{\small{Significance of E/B-modes for PSFz systematics. The first 20 COSEBIs modes are used to measure the E/B-modes. The significance is shown as a p-value for each angular range. }}
\label{tab:pvaluePSFz}
\begin{tabular}{  c  c  c  c   }
%   \cline{2-7}
                  & $[0.5',40']$        &  $[0.5',100']$         &  $[40',100']$           \\
  \hline
      no z-cuts, E-modes &  3.25e-01 & 2.08e-01 & 4.92e-01 \\
      no z-cuts, B-modes &  8.94e-01 & 5.54e-01 & 3.97e-01\\
  \hline
  single z-bin, E-modes & 7.78e-01 & 3.11e-23 & 1.65e-01\\
  single z-bin, B-modes &  2.95e-01 & 1.19e-08 & 4.48e-02\\
  \hline
  4 z-bins, E-modes & 3.40e-01 & 2.22e-93 & 5.51e-04\\
  4 z-bins, B-modes & 8.11e-01 & 1.37e-81 & 6.33e-04\\
\end{tabular}
\end{table}
 
 
 
 \subsection{B-modes in data and comparison to mock systematics}
 %Make a few comparison plots and one plot/table that shows there is b-modes. refer to the appendix for the other plots. 
 \begin{figure*}
   \begin{center}
     \begin{tabular}{c}
     \resizebox{180mm}{!}{\includegraphics{plots/weightedAllSurveys_EnBn_withTheory_1Bin_nMin1_nMax20_Npair_Input_weighted.pdf}}
     \end{tabular}
   \end{center}
     \caption{\small{COSEBIs E/B-modes for a single bin for three sets of public data. E-modes are shown on the left while B-modes are on the right panels. DES-SV data is shown with blue squares, KiDS-450 with black stars and CFHTLenS with magenta triangles. The angular ranges are shown for each row on the top right corner. In addition, the significance of the B-modes is shown as p-values for each survey and angular range. The errorbars solely show the noise contribution. For each survey theory E-mode values are calculated using the best fitting cosmological parameter values given in \tab\ref{tab:CosmoParam}. Note that COSEBIs modes are discrete and the theory values are connected to each other for visual aid. The red solid lines show the zero line, the blue solid, black dashed and magenta dotted curves belong to DES-SV, KiDS-450 and CFHTLenS, respectively. }}
     \label{fig:COSEBIsdata1bin}
 \end{figure*}
 
 
 
Finally in this section we show measurements of COSEBIs and CCOSEBIs for the data sets described in \sect\ref{sec:Data}. For the traditional statistics (2PCFs) see \App\ref{sec:AppData}. \fig\ref{fig:COSEBIsdata1bin} shows COSEBIs measurements for a single bin encompassing the full range of redshifts used in each dataset accordingly. We show results for the same angular ranges as in the previous sections. Each row corresponds to one angular range denoted in the right panels. DES-SV data is shown with blue squares, KiDS with black stars and CFHTLenS with magenta triangles. The E-modes are shown on the left panels, while B-modes are on the right. The errorbars on both panels only show the noise part of the covariance as described in \sect\ref{sec:Cov} and take into account the exact weighted number of galaxy pairs in each dataset. As a result, the E-mode errorbars are underestimated, however the B-mode errorbars are as accurate as possible. Although COSEBIs modes are discrete
we show the theory values for E-modes as curves, for ease of comparison. The theory values are calculated using the best fitting cosmological parameters of each survey (see \tab\ref{tab:CosmoParam}) and their corresponding redshift distribution. 
The significance of the B-modes are shown in the right hand panels for each dataset and angular range, using p-values. The p-value is equal to the probability of randomly producing the data, given the model. Here the model is that B-modes are equal to zero and their distribution is Gaussian, an assumption that holds for B-modes generated from noise. We see that the B-mode of KiDS-450 and CFHTLenS are consistent with zero, while DES-SV show significant B-modes with small p-values, when the full angular range is considered. This is consistent with the results shown in \cite{asgari/etal:2017} for CFHTLenS who used the first seven COSEBIs modes. Note that the COSEBIs modes are correlated to their neighbouring modes \citep[see][for plots of the covariance matrices]{Asgari12, asgari/etal:2017} and $\chi$ by eye should be avoided. For the E-modes we generally expect to see signal at the lower modes and none for the higher ones. This is due to the fact that both the 2PCFs and shear power spectrum are relatively smooth functions with a few features that are captured by the first few COSEBIs modes. The higher COSEBIs modes are sensitive to smaller angular range changes in the 2PCFs, which do not exist in the theory curves. 
 
One feature that stands out in the B-modes in \fig\ref{fig:COSEBIsdata1bin} is the high n-mode oscillatory pattern  in the full angular range shown in the middle panel.  All three datasets follow a very similar pattern which is closets to a regular pattern systematic case. The pointing shape and size of KiDS-450 and CFHTLenS are similar (squares of $\sim 1$ deg$^2$), however they are very different from DES-SV with a hexagonal pointing of 2.2 degrees across. Hence we do not expect this to be a pointing level regular pattern, but could still be due to a more fundamental effect, either to do with atmospheric effects or perhaps an astrophysical signal. {\color{red} now that KiDS and CFHTLenS dont have B-modes need to rephrase this.}  
 
The number of redshift bins and their range is different for each dataset. We show COSEBIs results for their corresponding redshift bins discussed in \sect\ref{sec:Data}, in \App\ref{sec:AppData}. Here we only show the significance of the B-modes in terms of p-values for each dataset and angular range in \tab\ref{tab:pvalue}. The p-values that are smaller than $0.01$ are shown in bold.
As can be seen from the table, KiDS-450 shows no significant B-modes, in contrast to previous analysis. Although we use a different statistic here that is sensitive to different parts of the data, we note that the main reason for this inconsistency is the corrections that we have done to the covariance matrix. Using the same prescription as the previous analysis to approximate the covariance matrix we also see B-modes in KiDS-450 data. On the other hand CFHTLenS shows hints of B-modes specially at smaller scales in contrast to \cite{asgari/etal:2017}. The main differences between the current work and \cite{asgari/etal:2017} is the addition of higher n-modes to the analysis and a more accurate covariance matrix that captures the geometry and variability of source densities in the images. These effects tend to enlarge the covariance at large scales where there are fewer pairs of galaxies due to geometry effects and decrease it for smaller scales where variable depth and source clustering become important. As a result the significance of the B-modes have decreased for large scales while they have become more significant for smaller scales. In addition, DES-SV data shows very significant B-modes, between $4\sigma$ and $6\sigma$ detection. This is in contrast to \cite{Becker15} who used power spectra to separate E/B-modes and concluded that the B-modes are insignificant. Power spectra pick up feature of the data at different scales to $\xi_\pm$ which form the primary observables in the main cosmic shear analysis of DES-SV. Therefore, an E/B-mode decomposition in the Fourier cannot accurately inform about real space quantities. This is in addition to the limitations of power spectrum methods. 

\begin{table}
\centering
\caption{\small{ Significance of B-modes for data. The first 20 COSEBIs modes are used to measure the B-modes in each dataset. The significance is shown as a p-value for each angular range. The single bins encompass all the galaxies used in the tomographic cases. All p-value that are smaller than $0.01$ are shown in bold. }}
\label{tab:pvalue}
\resizebox{\columnwidth}{!}{
\begin{tabular}{  c  c  c  c   }
%   \cline{2-7}
                  & $[0.5',40']$        &  $[0.5',100']$         &  $[40',100']$           \\
  \hline
      DES-SV, \;\;\; Single bin&  $4.86e-02$       & $\boldsymbol{2.59e-03}$             & $2.56e-02$\\
      DES-SV,       Tomography &  $\boldsymbol{9.94e-07}$       &   $\boldsymbol{1.53e-08}$           & $\boldsymbol{3.80e-05}$\\
  \hline
  	 KiDS-450,\;\;\; Single bin & $4.04e-01$      & $1.21e-01$             & $5.45e-01$\\
  	 KiDS-450,       Tomography & $9.35e-01$      & $6.07e-01$             & $7.71e-01$\\
  	 \hline
  	 CFHTLenS,\;\;\; Single bin & $6.29e-01$      & $6.07e-01$            & $5.75e-01$\\
  	 CFHTLenS,       Tomography & $\boldsymbol{2.51e-03}$      & $4.72e-02$            & $3.65e-02$\\
\end{tabular}
}
\end{table}


To get a better understanding of what sort of effect the systematics seen in the data can have on cosmology, we turn to CCOSEBIs. \fig\ref{fig:CCOSEBIsdata} shows the compressed COSEBIs modes that are sensitive to $\sigma_8$ and $\Om$.  The CCOSEBIs modes are highly correlated since  $\sigma_8$ and $\Om$ are degenerate in cosmic shear data. We use the same symbols and colours as in \fig\ref{fig:COSEBIsdata1bin} and the same three angular ranges. The empty symbols show the E-mode signal while the filled ones belong to B-modes. Theory E-mode signal is shown as curves for visual aid, although CCOSEBIs modes are discrete. The blue solid lines belongs to DES-SV, KiDS-450 is shown with black dashed lines and CFHTLenS with magenta dotted lines. The x-axis shows to which parameter (for the first order modes) or two parameters (for the second order modes) the CCOSEBIs mode is sensitive to. We use the redshift distribution and covariance matrix of each dataset to form the compression matrix, $\boldsymbol{\Gamma}$, for CCOSEBIs (see \sect\ref{sec:CCOSEBIs}). Note that once the compressed quantities that depend on second derivative of the observables are added, the efficiency of the compression is not sensitive to the exact form of the compression matrix as was shown in \cite{AS2014}. Hence we could have formed the compressed CCOSEBIs with less knowledge about the surveys, however, to find theory CCOSEBIs and their covariance we need to have this knowledge. Also note that as before the covariance matrix is for a noise only case and contain no cosmic variance terms. 

The left hand panel shows CCOSEBIs for the non-tomographic case. The left middle panel which has the highest signal to noise for the non-tomographic case can be compared to \fig\ref{fig:CCOSEBIsSys}. Based on that figure and the systematics that we have simulated a positive B-mode signal in CCOSEBIs for the angular range, $[0.5',100']$, corresponds to an increased $\Sigma_8$ measurement. Here we see that KiDS-450 shows the largest B-modes of the three datasets for this angular range. Following the above argument, we would expect the $\Sigma_8$ value estimated from KiDS-450 to be overestimated, which would increase its "discrepancy" with Planck lowP+TT results \citep[][]{Planck15}. Since CCOSEBIs modes are formed from those linear combinations of COSEBIs that are most sensitive to cosmological parameters, they are mostly based on the first few modes of COSEBIs. 

We compress the large data vectors for the tomographic cases\footnote{DES-SV with 3 redshift bins has 120 data points, KiDS-450 with 4 redshift bins has 200 data points and finally CFHTLenS with 6 redshift bins has 420 data points} into the same 5 CCOSEBIs modes and show the results in the right hand panels of \fig\ref{fig:CCOSEBIsdata}. We show the E-modes to compare with the level of B-modes and see that aside from the largest angular range with lowest signal-to-noise ratio, the E-modes are about an order of magnitude larger. In all panels we see that KiDS-450 signal is lower. This is due to the high redshift cut in this dataset. Both DES-SV and CFHTLenS have a higher mean redshift distribution compared to KiDS-450 (see \sect\ref{sec:Data}). 

\begin{figure*}
   \begin{center}
     \begin{tabular}{c}
     \resizebox{70mm}{!}{\includegraphics{plots/weightedCCOSEBIs_EBmodes_1bin_withTheory.pdf}}
     \resizebox{70mm}{!}{\includegraphics{plots/weightedCCOSEBIs_EBmodes_tomo_withTheory.pdf}}
     \end{tabular}
   \end{center}
     \caption{\small{CCOSEBIs E/B-modes for three public datasets for the non-tomographic (left) and tomographic (right) cases. The empty and filled symbols show E and B-modes, respectively. DES-SV data is shown with blue squares, KiDS-450 with black stars and CFHTLenS with magenta triangles. Three angular ranges are shown here, denoted at the top right corner of the right panels. The CCOSEBIs mode is indicated on the x-axis. The single parameters show the first order and the double parameters show the second order CCOSEBIs. All three datasets share the same compression matrix for the non-tomographic case. The errorbars only show the noise contribution.{\color{red} Change DES-SV m and z bias for single bin, hence theory.}}}
     \label{fig:CCOSEBIsdata}
 \end{figure*}



